Analysis and Control of Power-Temperature Dynamics in Heterogeneous Multiprocessors

Virtually all electronic systems try to optimize a fundamental trade-off between higher performance and lower power consumption. The latter becomes critical in mobile computing systems, such as smartphones, which rely on passive cooling. Otherwise, the heat concentrated in a small area drives both the junction and skin temperatures up. High junction temperatures degrade the reliability, while skin temperature deteriorates the user experience. Therefore, there is a strong need for a formal analysis of power consumption-temperature dynamics and predictive thermal management algorithms. This paper presents a theoretical power-temperature analysis of multiprocessor systems, which are modeled as multi-input multi-output dynamic systems. We analyze the conditions under which the system converges to a stable steady-state temperature. Then, we use these models to design a control algorithm that manages the temperature of the system without affecting the performance of the application. Experiments on the Odroid-XU3 board show that the control algorithm is able to regulate the temperature with a minimal loss in performance when compared to the default thermal governors.

==> files/sidebars_csm.tex <==
\subsection[Illustration]{Sidebar: Illustration of thermal fixed points}
\begin{figure}[h]
	\vspace{-1mm}	
	\centering
	\includegraphics[width=0.6\linewidth]{figures/motivation_new.pdf}
	\vspace{-1mm}
	\caption{
		Illustration of the power consumption temperature trajectory for two 
		power consumption levels using
		experiments performed on Odroid XU3 board~\cite{ODROID_Platforms}.} 
		%hat is 
	%powered by Samsung Exynos 5422 SoC. }
	\vspace{-2mm}
	\label{fig:motivation}
\end{figure}


To illustrate the problem addressed by this article, 
the power-temperature profile of a commercial SoC 
for a complete heat-up/cool-down cycle is measured, as shown in 
Figure~\ref{fig:motivation}.
First, the system starts with a power consumption of about 0.2~W. Then, the 
dynamic activity is increased so that the power consumption increases to 
0.9~W. As 
a result of the increase in power, the temperature rises quickly, denoted 
by segment marked as ``1''.
After this initial period, the dynamic activity of the system is kept at a 
constant level. Even though the dynamic activity is constant, the temperature 
keeps increasing towards a fixed point (segment 2). It is also seen that there 
is a corresponding increase in the power consumption of the system. This can be 
attributed to the increase in leakage power caused by the increase in the 
temperature. Eventually, the power-temperature dynamics reaches a steady state 
value given by (1.2~W, 69$^\circ$C). Once the steady state is reached, the 
dynamic activity is reduced and the power consumption of the system drops. This 
causes the temperature to decrease along segments 3 and 4, respectively. The 
existence of the fixed point alone is not sufficient to ensure thermally safe 
operation of the system. For example, when a higher dynamic activity is used, 
the trajectory converges to (2.6~W, 93$^\circ$C), which is larger than than the 
temperature which triggers throttling. Excessive throttling deteriorates the 
performance of the device and affects user experience. Therefore, runtime 
predictions of the fixed point temperature helps in taking effective dynamic 
thermal and power management decisions.


